Contrastive Vision-Language Alignment Makes Efficient Instruction Learner

We study the task of extending the large language model (LLM) into a vision-language instruction-following model. This task is crucial but challenging since the LLM is trained on text modality only, making it hard to effectively digest the visual modality. To address this, existing methods typically train a visual adapter to align the representation between a pre-trained vision transformer (ViT) and the LLM by a generative image captioning loss. However, we find that the generative objective can only produce weak alignment for vision and language, making the aligned vision-language model very hungry for the instruction fine-tuning data. In this paper, we propose CG-VLM that applies both Contrastive and Generative alignment objectives to effectively align the representation of ViT and LLM. Different from image level and sentence level alignment in common contrastive learning settings, CG-VLM aligns the image-patch level features and text-token level embeddings, which, however, is very hard to achieve as no explicit grounding patch-token relation provided in standard image captioning datasets. To address this issue, we propose to maximize the averaged similarity between pooled image-patch features and text-token embeddings. Extensive experiments demonstrate that the proposed CG-VLM produces strong vision-language alignment and is an efficient instruction learner. For example, using only 10% instruction tuning data, we reach 95% performance of state-of-the-art method LLaVA [29] on the zero-shot ScienceQA-Image benchmark.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{fig/FTdata_vs_SQAacc.pdf}
    % \vspace{-10pt}
    \caption{Comparisons to state-of-the-art visual instruction methods on zero-shot ScienceQA~\cite{lu2022sqa} image set \wrt~different amount of instruction tuning data. 
    }
    \label{fig:fig1}
    % \vspace{-17pt}
\end{figure}

Visual instruction-following model has been considered as the bedrock for the general-purpose assistant~\cite{li2023blip,dai2023instructblip} due to its ability to understand vision-language information and follow language instruction, drawing a large amount of attention from researchers~\cite{li2023blip,dai2023instructblip,gao2023llama,zhang2023llama,zhu2023minigpt,liu2023visual,liu2023improved,lin2023learning,chen2023a2nav}. Early attempts at vision instruction following models are restricted to image captioning~\cite{vinyals2016show,johnson2016densecap} and visual question answering~\cite{li2019visualbert,lu2019vilbert} tasks, limiting their application scenarios such as open-ended vision-language assistant~\cite{zhang2023llama}. Recently, attracted by the appealing instruction-following ability of large language models (LLM)~\cite{ouyang2022training,touvron2023llama,chiang2023vicuna}, researchers turn to adapt the LLM into a vision-language instruction following models, with the help of pre-trained vision transformer (ViT)~\cite{dosovitskiy2020image} from CLIP~\cite{alec2021clip}. The main focus is on how to combine the pre-trained ViT and LLM in order to complete the complex visual instruction task. 

To this end, existing methods often require a vision-language alignment step or mechanism that aligns the vision and text modalities by learning a visual adapter. There are mainly two lines of work: heavyweight adaptation~\cite{li2023blip,zhu2023minigpt,dai2023instructblip,alayrac2022flamingo,bai2023qwen} and lightweight adaptation~\cite{gao2023llama,zhang2023llama,liu2023visual,liu2023improved}. BLIP-2~\cite{li2023blip}, MiniGPT4~\cite{zhu2023minigpt} and InstructBLIP~\cite{dai2023instructblip} leverage a heavy visual adapter Q-former, a BERT~\cite{kenton2019bert} model, to align different modalities. Flamingo~\cite{alayrac2022flamingo} propose to use perceiver~\cite{jaegle2021perceiver} and gated xattn-dense layers to respectively extract and inject vision-language features into a pre-trained Chinchilla LLM~\cite{hoffmann2022training}. Different from them, lightweight adaptation methods such as LLaMA-Adapter~\cite{gao2023llama,zhang2023llama} and LLaVA~\cite{liu2023visual,liu2023improved} propose to learn a linear or MLP projector that connects the pre-trained ViT and LLM. During the vision-language alignment step, the visual features from ViT are projected to the embedding space of LLM by the visual adapter. Then, the projected visual features are fed into LLM and are optimized by the image captioning loss in a generative (\ie auto-regressive) way.

% \begin{table}[!t]
%     \centering
%     \resizebox{0.8\linewidth}{!}{\small
%         \begin{tabular}{l|cr}
%         % \toprule
%         \hline
%         Method & Align Type & Top-1 Acc. (\%) \\
%         \hline\hline
%         \textcolor{gray}{CLIP}~\cite{alec2021clip} & \textcolor{gray}{Con} & 
%         \textcolor{gray}{69.03} \\
%         \hline
%         LLaVA~\cite{liu2023improved} & Gen & 0.14 \\
%         % CTC (Ours) & Con & 21.74 \\
%         CTC (Ours) & Con + Gen & 13.61 \\
%         % \without & \without & 44.2 & 61.8 & 52.9 & 64.9 \\
%         % \hline
%         % \with & \without & \noimprove{41.6}{2.6} & \noimprove{58.6}{3.2} & \noimprove{51.1}{1.8} & \noimprove{63.6}{1.3} \\
%         % \with & \with & \bestimprove{52.2}{6.7} & \bestimprove{63.8}{2.0} & \bestimprove{59.3}{6.4} & \bestimprove{66.3}{1.4}\\
%         % \bottomrule
%         \hline
%         \end{tabular}
% }
% \caption{Zero-shot evaluation on ImageNet using the text prompt template \texttt{A photo of a \{class name\}}. Con and Gen are short for Contrastive and Generative, respectively.}
% \label{tab:imgnet_cls}
% \end{table}

However, we suspect that training the visual adapter in a generative manner may not align vision-language modalities effectively. To verify this, we visualize the cosine similarities between the image patch and text token, and the results are shown in Figure~\ref{fig:motivation}. We find that the text token features often have a large cosine similarity to a majority of vision patch features, showing the weak alignment between vision-language modalities. Moreover, this weak alignment makes the model very data-hungry for the vision instruction fine-tuning data. From Figure~\ref{fig:fig1}, with a generative aligned visual adapter, the accuracy of state-of-the-art method LLaVA~\cite{liu2023improved} on Science-QA~\cite{lu2022sqa} image set drops significantly as the amount of instruction tuning samples decreases. On one hand, instruction tuning data is very crucial for generalization to vision-language tasks~\cite{dai2023instructblip}. On the other, high-quality instruction data is very hard to collect since the process is time-consuming and less well-defined when human crowd-scouring is considered~\cite{liu2023visual}. In this sense, how to align the vision language effectively remains an important but unsolved question.  
% \lec{Emphasize the importance of instruction data efficiency. Collecting high-quality instruction data is very difficult.}

% we use ImageNet~\cite{deng2009imagenet} zero-shot probing accuracy like CLIP~\cite{alec2021clip} to evaluate the vision-language alignment quality. As shown in Table~\ref{tab:imgnet_cls}, the zero-shot probing accuracy of the generatively-trained visual adapter is near random guesses. Moreover, as depicted in Figure~\ref{fig:motivation}, the cosine similarity map between vision patch features and text token features also shows weak alignment between vision-language modalities. Last but not least, this weak alignment makes the model very data-hungry for the vision instruction fine-tuning data. As shown in Figure~\ref{fig:fig1}, with a generative-only aligned visual adapter, the accuracy of Science-QA~\cite{lu2022sqa} image-related questions drops significantly.

\begin{figure*}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{fig/motivation.pdf}
    \caption{Comparisons of the image features projected by different visual adapters. With generative objective only, the projected visual features of LLaVA~\cite{liu2023improved} have large similarities to all visual concepts. In contrast, with the proposed contrastive and generative aligned visual adapters, our \shortname provides \textit{only} large similarities to the corresponding concepts.\protect\footnotemark
    }
    \label{fig:motivation}
    % \vspace{-10 pt}
\end{figure*}

In this paper, we propose \name (\shortname) to effectively align the vision-language modalities from pre-trained ViT and LLM. To be specific, we use contrastive loss to align the vision and text features from the visual adapter and LLM embedding layer, respectively. 
However, as the averaged token embeddings of LLM layers are very ambiguous among different sentences~\cite{ethayarajh2019contextual}, 
% However, 
how to align the visual features to a sequence of token embeddings from the caption remains an unknown question. To this end, we propose to average the similarities between pooled image features and token features from one sentence as the image-sentence similarities. Then, we optimize the image-text similarities from batch data like CLIP~\cite{alec2021clip}. Though the proposed contrastive objective provides better vision-language alignment performance, the average mechanism of image-sentence alignment inevitably focuses on the dominant visual concepts, resulting in sub-optimal vision-language alignment of the nondominant concepts or semantics. To address this issue, we preserve the original generative objective that should attend to the detailed and rich visual concept in order to complete the dense image captioning task. With our proposed \shortname, we make better visual instruction tuning in two aspects: \textbf{1)} a visual instruction tuning data efficient vision-language model that achieves most of the performance even trained with only 10\% amount of the original data. \textbf{2)} preserves more text ability from the original LLM and achieves better results on the text-only instruction or question. We summarize our main contributions as follows:
\begin{itemize}
    \item To the best of our knowledge, we are the first to analyze the vision-language representation alignment issue in the visual instruction tuning task and find that existing works can not effectively align vision-language with only the generative objective given limited instruction tuning data. 

    \item To effectively align vision-language modalities, we propose to use the contrastive objective on the image-sentence similarities. Moreover, to remedy the sub-optimal alignment of non-dominant concepts, we also preserve the original generative objectives to focus more on the rich and detailed semantics.

    \item Extensive experiments on popular visual question answering and human instruction following benchmarks show that the proposed \shortname surpasses the baseline method by a large margin under the instruction efficient settings and achieves competitive results compared to methods that use 100$\times$ instruction tuning data. 
\end{itemize}

==> sec/4_experiments.tex <==
\section{Experiments}

\invisiblesection{Pre-training and fine-tuning datasets} 
We construct datasets for two stages: vision-language pre-training and visual instruction tuning, as done in previous works~\cite{liu2023visual,liu2023improved,dai2023instructblip,bai2023qwen}. For the pre-training stage, we leverage the LCS-558K dataset, a subset of about 558K image-text pairs from LAION-CC-SBU~\cite{schuhmann2021laion}. 
For the visual instruction tuning stage, we randomly shuffle the 665K instruction-following datasets created by LLaVA 1.5~\cite{liu2023improved} and preserve only 1\% and 10\% data to validate the model's performance under limited curated instruction-following data.\footnote{More details on the sub-sampled datasets are put in the supplementary.}
% For the visual instruction tuning stage, we fine-tune the language model on the 665K mixture of multi-task instruction-following datasets created by LLaVA 1.5~\cite{liu2023improved}. 
% For experiments on efficient instruction settings, we randomly shuffle the 665K instruction-following datasets and preserve only 1\% and 10\% data, resulting in two additional subsets with 6K and 66K data.\footnote{More details on the sub-sampled datasets are put in the supplementary.}
% We evaluate our \shortname on ScienceQA and COCO Caption benchmarks

\invisiblesection{Implementation details} We use the vision transformer of CLIP ViT-L/14~\cite{alec2021clip} and Vicuna 13B~\cite{chiang2023vicuna} to instantiate our pre-trained ViT and LLM, respectively. For text-only questions, a blank image is inputted as the placeholder into the vision transformer. During the vision-language pre-training stage, we only learn the visual adapter by freezing the parameters of pre-trained ViT and LLM. For visual instruction tuning, we only freeze the pre-trained ViT while tuning all other modules. Following the common practice of previous works~\cite{liu2023visual,liu2023improved}, the learning rate for pre-training and fine-tuning is $1\text{e}^{-3}$ and $2\text{e}^{-5}$, respectively. We use a cosine learning rate scheduler with a 0.03 warmup ratio. For both pre-training and fine-tuning, we only run through the dataset for 1 epoch. We set the penultimate visual patch features of ViT as the input for the visual adapter. The default architecture for the visual adapter is an MLP module with two linear layers and GELU~\cite{hendrycks2016gaussian} activation function.
% The batch size for pre-training and fine-tuning are set to 32 and 16 per GPU, respectively. 
The optimization strength of contrastive loss $\alpha$ is set to 1.0 default. For the LLaVA baseline and our \shortname, we fine-tune them on 66K instruction tuning data by default. All experiments are conducted on an 8$\times$A800 machine.\footnote{More implementation details can be found in the supplementary.}


\subsection{Comparison with State-of-the-arts}
To investigate the visual perception, visual-language understanding and reasoning ability of the proposed \shortname, we conduct extensive experiments on three kinds of benchmarks, namely, image captioning, visual question answering, and instruction-following.

% We evaluate our \shortname on various multi-modal tasks to investigate the visual perception and visual-language understanding ability. Specifically, we perform three types of multi-modal tasks: image captioning, visual question answering, and instruction-following.

\begin{table}[t]
\centering
\small
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{@{}lr|cc@{}}
\toprule
Method                                 & \begin{tabular}[c]{@{}c@{}}\#Instruction\\ Tuning Data\end{tabular} & MME    & SEED \\ \midrule
BLIP2~\cite{li2023blip}                 & -    & 1293.8 & 46.4 \\
MiniGPT4~\cite{zhu2023minigpt}          & -    & 581.7  & 47.4 \\
InstructBLIP~\cite{dai2023instructblip} & 1.2M & 1212.8 & 58.8 \\
% Shikra~\cite{chen2023shikra}            & \sxy{?}  & -      & -    \\
LLaMA-AdapterV2~\cite{gao2023llama}     & 50M  & 972.7  & 35.2 \\
LAVIN~\cite{luo2023cheap}               & 210K & 963.6  & -    \\
LLaVA~\cite{liu2023llava}               & 158K & 502.8  & 37.0 \\
mPLUG-Owl~\cite{ye2023mplug}            & 392K & 967.3  & 37.9 \\
Qwen-VL-Chat~\cite{bai2023qwen}         & 50M  & 1487.5 & 65.4 \\ \midrule
LLaVA-1.5~\cite{liu2023improved}        & 66K  & 1061.8 & 51.1 \\ 
\shortname (Ours)                       & 66K  & \textbf{1318.2} & \textbf{60.9} \\ \midrule
LLaVA-1.5~\cite{liu2023improved}        & 6K   & 1051.8 & 45.3 \\ 
\shortname (Ours)                       & 6K   & \textbf{1143.2} & \textbf{51.4} \\ \bottomrule
% LLaVA-1.5~\cite{liu2023improved}        & Vicuna-13B & 1531.3 & 61.6 & 67.7    & 63.4        \\ \midrule
% \shortname (Ours)                       & Vicuna-13B &        &      &         &             \\ \bottomrule
\end{tabular}}
% \vspace{-5pt}
\caption{Comparisons with state-of-the-art visual instruction tuning methods on human instruction-following benchmarks.}
\label{tab:sota-ins}
\end{table}

% Please add the following required packages to your document preamble:
\begin{table}[t]
\small
\centering
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{@{}ll|ccc@{}}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Alignment\\ Objective\end{tabular}} & \multicolumn{2}{c}{ScienceQA} & \multirow{2}{*}{POPE} \\ \cmidrule(lr){3-4}
                        &                                                                                & Text        & Image       &                       \\ \midrule
LLaVA~\cite{liu2023improved}  & Gen.                                                                           & 73.7        & 62.4        & 81.3                  \\
\multirow{2}{*}{\shortname}    & Con.                                                                           & 72.2        & 59.7        & 80.9                  \\
                        & Con.+ Gen.   & ~~~~~~~\bestimprove{77.0}{3.3}                     & ~~~~~~~\bestimprove{67.4}{5.0}                      & ~~~~~~~\bestimprove{85.4}{4.1}                  \\ \bottomrule
\end{tabular}}
% \vspace{-5pt}
\caption{Ablation studies on different alignment objectives. Both LLaVA and our CG-VLM are trained on the 10\% subset of instruction-tuning data. Gen. and Con. are short for Generative and Contrastive, respectively.}
\label{tab:ablation-align}
\end{table}

\invisiblesection{Results on visual question answering} We first evaluate our model on the object probing dataset (POPE~\cite{li2023pope}). In this task, the vision-language model is asked to answer a series of questions about the existence of specific objects in the image. From the first column in Table~\ref{tab:sota-vq}, we found that our \shortname model produced more accurate probing results since it is well-trained to distinguish objects through image-text paired contrastive learning. Using only 6K instruction tuning data, our \shortname model surpasses InstructBLIP trained on a much larger data scale (80.0 \vs 78.9), which shows the effectiveness of contrastive alignment for accurate perception and less object hallucination.
% preventing the model from the object hallucination problem.
% Additionally, to verify whether our VLM model suffers from the object hallucination problem, we further adopt a polling-based query benchmark POPE~\cite{li2023pope} to examine our \shortname model.

We further test our model on another two variants of the visual question-answering benchmarks, including text-oriented VQA and general VQA benchmarks. For text-oriented VQA benchmarks, we adopt TextVQA~\cite{singh2019textvqa} which requires the VLM model to read the text within images and reason the answers. For general VQA, we utilize three benchmarks various from VQAv2~\cite{goyal2017vqav2}, GQA~\cite{hudson2019gqa} to ScienceQA~\cite{lu2022sqa} to examine visual perception and reasoning ability. We report direct comparison results with a generative pre-training baseline (LLaVA-1.5) under two different data fractions, 6K and 66K. Overall performance on all VQA tasks is reported in Table~\ref{tab:sota-vq}. As the results show, our \shortname significantly improves the model's ability among all VQA tasks. It is worth noting that on the GQA benchmark, which consists of complex compositional questions, our \shortname achieves 54.0\% overall accuracy when finetuned on 66K instruction data, compared to 40.7\% of the baseline model. We attribute it to our alignment objective. By explicitly reducing the modality gap between visual and language inputs during the pre-training stage, it enables accurate perceiving and reasoning of objects in the image.

\invisiblesection{Results on instruction-following} For modern VLM models, the ability of instruction-following is crucial and of essential concern in real-world scenarios where diverse commands will be encountered. To investigate our \shortname model's performance in this scenario, we conduct evaluations on the MME~\cite{fu2023mme} and SEED~\cite{li2023seed} benchmarks. We report the perception score for the MME benchmark. For the SEED benchmark, we report accuracy on the image set. Results are shown in Table~\ref{tab:sota-ins}.
Despite extremely little training data, our \shortname still yields better results on both MME and SEED benchmarks, compared with previous methods trained on much larger datasets (\ie InstructBLIP and LLaMA-AdapterV2). We also achieved competitive performance against the data-hungry method Qwen-VL-Chat (1318.2 \vs 1487.5), which is trained on 1.4B image-text pairs and 50M multi-task instruction data. These results demonstrate that \shortname is able to adapt rapidly to a small amount of instruction tuning data while preserving strong generalization ability to unseen instructions.
% demonstrates competitive performance against methods that trained on heavy instruction tuning datasets (\ie, Qwen-VL-Chat that trained on 50M data, ours 66K) 

\subsection{Ablation Analysis on \shortname}
% \vspace{-5pt}
We conduct ablation studies to investigate the effectiveness of different alignment objectives: generative-only (LLaVA~\cite{liu2023improved}) and using both contrastive and generative objectives (our \shortname). The POPE~\cite{li2023pope} and ScienceQA~\cite{lu2022sqa} benchmarks are selected to evaluate the abilities of visual perception, visual-language reasoning and language-only reasoning. The results are shown in Table~\ref{tab:ablation-align}. Compared to the generative objective, using the contrastive objective only leads to performance degradation on all metrics, showing that discarding the generative objective totally to learn vision-language alignment is not feasible, especially when no explicit grounding information is provided for image-patch and text token. Instead, our \shortname combines both contrastive and generative objectives, which not only directly aligns the dominant visual concepts effectively, but also aligns the non-dominant ones supervised by the generative loss. From Table~\ref{tab:ablation-align}, we observe remarkable improvements in both datasets after pre-training using our proposed contrastive alignment objective. Specifically, for visual perception ability, \shortname improves the results on POPE dataset by 4.1\%. For vision-language understanding, we observe improvements in both visual (67.4 \vs 62.4) and text (77.0 \vs 73.7) modalities on the ScienceQA dataset. These findings support the superiority of using both contrastive and generative objectives other than generative only.

% \invisiblesection{Effectiveness of soft prompt tuning}


% \subsection{Further Analysis on \shortname}
% To gain deeper insights into our \shortname, we further conduct a series of ablation studies of the detailed design \sxy{during the instruction process}.


% \begin{table}
% \centering
% \small
% \begin{tabular}{@{}cc|cc@{}}
% \toprule
% Align method                & Tune proj.        & SciQA-IMG & POPE   \\ \midrule
% \multirow{2}{*}{LLaVA}      & \tiny\Checkmark   &  62.4     & 81.3  \\
%                             & \tiny\XSolidBrush &           &      \\ \midrule
% \multirow{2}{*}{\shortname (Ours)} & \tiny\Checkmark   &  66.4     & 86.1 \\
%                             & \tiny\XSolidBrush &  67.4     & 85.4  \\ \bottomrule
% \end{tabular}
% \caption{Ablation studies on projector learning strategy.}
% \label{tab:ablation-proj-tune}
% \end{table}

\subsection{Further Analysis on \shortname}
% \vspace{-5pt}
\invisiblesection{Effect of $\alpha$ in Eqn.~(\ref{eqn:alignment_loss})}
Recall that $\alpha$ is used to control the optimization strength of contrastive loss in the vision-language alignment stage. We investigate its effect on the visual instruction-tuning performance of ScienceQA and POPE by setting $\alpha$ to 0.5, 1.0 and 2.0. From the results in Table~\ref{tab:ablation-alpha}, we observe our \shortname is relatively robust to the choices of $\alpha$ when $\alpha \geq 1.0$ and the best results are achieved when $\alpha=1.0$. When decreasing $\alpha$ to $0.5$, the performance on both ScienceQA and POPE drops substantially, indicating that strong optimization strength on the contrastive loss is important to achieve better performance.

\invisiblesection{Effect of projector design} Since the projector is optimized to minimize both generative and contrastive objectives, we are curious about its capacity. We investigate the capacity of the projector by instantiating it into an MLP layer or a linear layer and the results are shown in Table~\ref{tab:ablation-proj-design}. We find that using the MLP projector achieves the best results, indicating that an adapter with strong learning capacity is able to facilitate the vision-language alignment process.

\begin{table}[t]
\centering
\small
\begin{tabular}{r|ccc}
\toprule
$\alpha$  &  0.5  & 1.0  & 2.0 \\ \midrule
SciQA-IMG &  64.5 &  \textbf{67.4} & 67.1    \\
POPE      &  84.4 &  \textbf{85.4} & \textbf{85.4}    \\ \bottomrule
\end{tabular}
% \vspace{-5pt}
\caption{Ablation studies on $\alpha$ in Eqn.~(\ref{eqn:alignment_loss}).}
\label{tab:ablation-alpha}
% \vspace{-5pt}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{r|cc}
\toprule
Projector Type & MLP & Linear \\ \midrule
SciQA-IMG      &  \textbf{67.4}     &  64.0 \\
POPE           &  \textbf{85.4}     &  81.0  \\ \bottomrule
\end{tabular}
% \vspace{-5pt}
\caption{Ablation studies on the projector type.}
\label{tab:ablation-proj-design}
% \vspace{-5pt}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{r|ccc}
\toprule
Ratio  & 1\% & 10\% & 100\% \\ \midrule
SciQA-IMG &  47.6 &  62.1 & 67.4    \\
POPE &  49.2 &  67.7 & 85.4    \\ \bottomrule
\end{tabular}
% \vspace{-5pt}
\caption{Ablation studies on different amounts of pre-trained data.}
\label{tab:ablation-pretrain-data}
% \vspace{-5pt}
\end{table}

\invisiblesection{Effect of pre-trained data amount} Although pre-trained data is much easier to obtain than the instruction tuning data, we are still curious about how the amount of pre-trained data affects the visual instruction-following performance. We conduct experiments by setting the amount of pre-trained data to 1\%, 10\% and 100\%. From the results in Table~\ref{tab:ablation-pretrain-data}, our \shortname achieves competitive results with only 10\% pre-trained data on the SciencQA image set, showing that \shortname has great potential for efficient vision-language alignment. 
% We also observed gradual improvement as the pre-training data scale rises. Since it is much easier to collect image-text pairs for pre-training, our approach holds significant promise as the scale of pre-training data expands.

% \invisiblesection{Logit scale} xxx

% \invisiblesection{Prompt length} xxx

% \invisiblesection{Text select layer}

% \invisiblesection{Original Text ability} xxx

% \invisiblesection{Sort Prompt Position} xxx

% \invisiblesection{Effect of Pretrain Batch Size} xxx

\subsection{Qualitative Results of \shortname} 
\vspace{-5pt}
To intuitively understand our \shortname's ability of visual perception, vision-language understanding and visual instruction-following, we provide visual comparison results between LLaVA 1.5~\cite{liu2023improved} and our \shortname in Figure~\ref{fig:visualization}. Note that both LLaVA 1.5 and \shortname are fine-tuned on the 10\% subset of data. We construct our test cases to evaluate the abilities of visual instruction models in three aspects.

\invisiblesection{Visual perception and reasoning ability} From the first column, we find that our \shortname accurately perceives and reasons about the visual concepts (``holding $\cdots$ clothing and possibly ironing it''), while LLaVA can not accurately capture relevant visual concepts and fails to understand the odd context in the image
% (``yellow pants'', ``holding a yellow umbrella'').
(``holding a yellow umbrella'').

\invisiblesection{Visual instruction-following ability} As shown in the top right, our \shortname understands the query and completes the required task based on rich visual details (``a light bulb in its beak'', ``Order yours today''), while LLaVA fails to follow instruction and only produces a caption-like response (``sitting next to a book and a cell phone''). 

\invisiblesection{Original LLM ability} As depicted in the bottom right, our \shortname preserves more original LLM ability and gives a detailed introduction of pandas (``native to China'', ``known for their $\cdots$''), while LLaVA can only roughly describe the image content (``in a zoon and in a tree'').

% \subsection{Comparison of data efficiency}
% As discussed in previous work~\cite{dai2023instructblip}\sxy{[TODO], the quality and amount of training data in the instruction tunning stage is crucial for VLM to master complex vision-language interaction.} We compare the visual question answering performance under different data scales in the instruction tunning stage and find out our \shortname is a data-efficient learner. \sxy{[TODO] (a chart)} We surprisingly observed that our \shortname surpasses most of the previous SOTA VLM models even though only 66K instruction-following data are available. \sxy{[TODO] (further analyses)}

==> sec/6_todo.tex <==
\section{TODO}
Inspired by the great success of unsupervised pertaining of vision transformers (ViT)~\cite{xxx} and large language models (LLM), early attempts~\cite{xxx} try to directly pretrained the multimodal transformers, hoping it generalizes well on a wide range of downstream tasks. CoCa~\cite{yu2022coca} trains the multimodal model from scratch with both contrastive and captioning objectives. Flanmingo~\cite{alayrac2022flamingo} xxxx. VisualBERT~\cite{li2019visualbert} treats both image and text as one modality and feeds it into transformer~\cite{xxx} to learn multimodal in a unified way. Although these methods achieve very competitive performance on multimodal tasks such as visual question answering~\cite{xxx}. They are inherently restricted to specialized domains or tasks, failing to tackle open-end scenarios such as multimodal instruction following models~\cite{xxx}.

However, direct optimization of multimodal models is very computationally intensive and time-consuming due to a great amount of image-language data and inherent modality gap~\cite{xxx}, resulting in huge resources consuming \eg (Flanmingo~\cite{alayrac2022flamingo} use xxx).

Recently, to obtain multimodal vision-language models in an efficient way, researchers propose to adapt the pretrained large language models with visual adaptation 
Early attempts such as BLIP-2~\cite{li2023blip} and xxx train a heavy visual adapter Q-former to align different modalities.
such as LLaMA-Adapter~\cite{zhang2023llama}, LLaMA-Adapter V2~\cite{gao2023llama}, LLaVA~\cite{liu2023visual}, LLaVA V2~\cite{liu2023improved} and MiniGPT-4~\cite{zhu2023minigpt} ... These kinds of methods typically introduce two stages \ie~visual-text alignment and visual-instruction tuning to combine the pretrained ViT and LLM into a multimodal instruction following model. To be specific, the visual-text alignment often applies the generative pertaining loss to train the visual adapter on the image captioning datasets. 

However, we find that training the visual adapter in this manner is not only training inefficient but also shows a weak alignment between the visual and text features. We argue that the weak alignment between two modalities impedes the performance of further visual instruction tuning stage.

If the ViT can be well comprehended by LLM, there is no need to use extra heavy resources to fine-tune the LLM, which may cause serious forgetting problems.

To find the best semantic granularity match, we use a linear weighted strategy to combine the cls features from different ViT and LLM hidden layers and apply the contrastive learning on the weighted average of the cls features.

%%%%%%%%%%%%%%%%%%%%%%%%%% TODO notes here %%%%%%%%%%%%%%%%%%%%%%%%%%
\sxy{[Writing]} In LLM layers, averaged token embeddings in different sentences can not be discriminated in the hypersphere feature space. (\sxy{Does CLIP possess this problem?}). For example, the sentence ``a photo of a boy" is similar to ``a photo of a woman". In the meantime, we observe that only token-level embeddings are discriminative in the feature space.

\sxy{[Writing]} Autoregressive-based pre-training makes aligning semantics in images and text hard.


\lec{[Writing]} GreenAI, reuses the computation power from the big corporation's institutes. Even with lots of resources, it will be hard to harvest detailed images to caption data for precise generative training. Our work can be seen as an efficient way to combine the models trained from abundant unimodal resources and connect them into a multimodal backbone in an efficient way.

\lec{[Writing]} Inspired by CLIP it bridges the language and vision signals, some pioneer works already use it for zero-shot image captioning.

\lec{[Writing]} Our method inserts the visual embedding in the middle LLM layers, which saves nearly half of the computation compared to feeding them into the LLM input end.

\lec{[Writing]} Full fine-tuning of the LLM may cause catastrophic forgetting.

\lec{[Writing]} With contrastive alignment, our CTC is able to condense the discriminative visual features into a relatively small region, paving the wave for using fewer visual tokens during fine-tuning.

\lec{[Writing]} The intuition of our multi-layer alignment is simple: compared to billions of text pretrain corpus and the drastic feature similarity changed across the LLM layers, the small-scale visual instruction data is not enough to fine-tune the LLM, making it treat the visual token as the textual one.

\lec{[Method]} To show the effectiveness of the proposed patch-token contrastive loss, we first use two simple baselines: 1) a pooled representation of the LLM hidden states and 2) a learnable [CLS] embedding. Unfortunately, two baselines both fail at convergence. To diagnose these issues, we measure the similarity between different sentences of the LLM hidden states and find that the pooled or [CLS] representation has a very high cosine similarity between them. In this sense, they are indistinguishable and therefore they can not be used as a learning target for contrastive alignment loss.

\lec{[Method]} We find that optimizing the averaged similarity between image descriptor and text representation leads to the dominant problem where only the most discriminative image concept is aligned while leaving other important concepts not aligned. To address this issue, we propose a masking strategy that masks some image tokens before performing average pooling, which provides chances for undominant concepts to be aligned.

\lec{[Experiment]} Verify the effectiveness of the contrastive alignment: Use a randomly initialized projector or contrastively aligned projector and see the convergence speed.

\lec{\underline{[Experiment]-Done}} Linear Probe on the imagenet data. For baseline, we use BoW as a linear classifier. As to our CTC which is contrastively aligned to the contextual embedding, we can use the sentence hidden states as the linear classifier.

\lec{\underline{[Experiment]-Done}} Visualize the similarity between image patch and text token embedding to demonstrate the learned similarity.

\lec{[Experiment]} Data-efficient settings, 1\%, 5\%, 10\%, 50\%, 100\% data, and achieve very competitive performance.

\lec{[Experiment]} LLaVA baseline, fine-tune it by freezing the llama model.

\lec{[Experiment]} Compare LLaVA and \shortname by freezing the projector.

\lec{[Figure]} Plot the contrastive alignment and soft-prompts fine-tuning in a single figure.

\lec{[Figure]} Compare chat results of LLaVA and \shortname trained by 1\%, 5\%, 10\%, 100\%.
